CoT-Kinetics: A Theoretical Modeling Assessing LRM Reasoning Process

Recent Large Reasoning Models significantly improve the reasoning ability of Large Language Models by learning to reason, exhibiting the promising performance in solving complex tasks. LRMs solve tasks that require complex reasoning by explicitly generating reasoning trajectories together with answers. Nevertheless, judging the quality of such an output answer is not easy because only considering the correctness of the answer is not enough and the soundness of the reasoning trajectory part matters as well. Logically, if the soundness of the reasoning part is poor, even if the answer is correct, the confidence of the derived answer should be low. Existing methods did consider jointly assessing the overall output answer by taking into account the reasoning part, however, their capability is still not satisfactory as the causal relationship of the reasoning to the concluded answer cannot properly reflected. In this paper, inspired by classical mechanics, we present a novel approach towards establishing a CoT-Kinetics energy equation. Specifically, our CoT-Kinetics energy equation formulates the token state transformation process, which is regulated by LRM internal transformer layers, as like a particle kinetics dynamics governed in a mechanical field. Our CoT-Kinetics energy assigns a scalar score to evaluate specifically the soundness of the reasoning phase, telling how confident the derived answer could be given the evaluated reasoning. As such, the LRM's overall output quality can be accurately measured, rather than a coarse judgment (e.g., correct or incorrect) anymore.

==> sections/backup.tex <==
% \subsection{Self-Evaluation via Discrete Semantic Action}
% \label{Problem Definition}


% We consider the setting where a LLM performs Chain-of-Thought (CoT) reasoning over a batch of input queries \(\{Q_i\}_{i=1}^B\).
% For each query, the model generates a reasoning trajectory and a final answer, denoted \((\mathrm{CoT}_i, A_i^{\text{LLM}})\), producing a set of prediction tuples \(\{(Q_i, \mathrm{CoT}_i, A_i^{\text{LLM}})\}_{i=1}^B\).
% Ground-truth answer labels \(\{A_i^{\text{GT}}\}_{i=1}^B\), where \(A_i^{\text{GT}} \in \{0,1\}\), are assumed to be available for evaluation.

% \begin{tcolorbox}[colback=blue!8!white, colframe=blue!40!black,
%   title=Problem Definition, fonttitle=\bfseries]

% The goal of \textbf{self-evaluation} is to equip the model with a decision function
% \[
% f: (Q_i, \mathrm{CoT}_i, A_i^{\text{LLM}}) \mapsto s_i \in \mathbb{R},
% \]
% which assigns a confidence score \(s_i\) to each prediction. A higher score should indicate a higher likelihood that the model's output is correct and its reasoning trajectory is reliable.

% \end{tcolorbox}

% The quality of the decision function is evaluated by comparing the score-induced ranking \(\{s_i\}\) against the binary correctness labels \(\{A_i^{\text{GT}}\}\), using three standard classification metrics.

% First, we compute \textbf{AUROC}, which measures the pairwise ranking consistency between positive and negative samples. Let \(\mathcal{P} = \{i \mid A_i^{\text{GT}} = 1\}\) and \(\mathcal{N} = \{j \mid A_j^{\text{GT}} = 0\}\). Then:
% \begin{equation}
% \text{AUROC} = \frac{1}{|\mathcal{P}||\mathcal{N}|} \sum_{i \in \mathcal{P}} \sum_{j \in \mathcal{N}} \mathbb{1}(s_i > s_j),
% \quad
% \text{FPR@95} = \frac{\mathrm{FP}_{@95}}{|\mathcal{N}|}.
% \end{equation}

% Second, we report \textbf{AUPR}, which quantifies the precision-recall tradeoff across different thresholds, based on the ranking induced by \(\{s_i\}\). Finally, \textbf{FPR@95} is the false positive rate when the true positive rate reaches 95\%, where \(\mathrm{FP}_{@95}\) denotes the number of negative samples incorrectly ranked above the 95th percentile of positive scores.





Let \( q_t \in \mathbb{R}^d \) denote the mean hidden state of reasoning-relevant tokens at layer \( t \in \{0, 1, ..., N\} \). The sequence \( \{q_t\}_{t=0}^N \) forms a semantic evolution in embedding space. This evolution is iteratively updated within each transformer layer:

\begin{equation}
q_{t+1} = f_t(q_t, A_t), \quad \text{for } t = 0, 1, \dots, N-1
\label{eq:trajectory}
\end{equation}

where \( f_t(\cdot) \) denotes the layer-specific transformation function, and \( A_t \) captures the attention-derived contextual information at layer \( t \). Equation~\ref{eq:trajectory} thus encodes the progressive construction of internal reasoning states, layer by layer.

The final answer is not directly generated from the input prompt \( x \) alone, but conditioned on the complete reasoning trajectory, including the CoT tokens generated during inference. Formally, the answer token \( y_{\text{ans}} \) is obtained by:

\begin{equation}
y_{\text{ans}} = \arg\max_y P(y \mid x, \text{CoT})
\label{eq:system2-decision}
\end{equation}

This formulation highlights the fundamental distinction of System 2 reasoning: the model's prediction relies on both the original prompt and an internally generated reasoning trajectory.

\subsection{Discrete Lagrangian Mechanics}

To evaluate the quality of each reasoning trajectory, motivated by classical mechanics, we propose to model reasoning trajectories in LLMs as discrete Lagrangian mechanics governed by Hamilton's principle.  
In physics, Hamilton's principle states that a system's physical trajectory is governed not merely by local forces, but by the accumulated behavior of the system's \emph{action} \(S\) over time.  
The action \(S\) is defined as the time integral of the Lagrangian \(L = T - U\), where \(T\) represents kinetic energy and \(U\) denotes potential energy:

\begin{equation}
S = \int_{t_1}^{t_2} L(q, \dot{q}, t) \, dt,
\quad L = T - U,
\end{equation}

Here, \(q\) is the system’s state variable, and \(\dot{q}\) is its time derivative, capturing the instantaneous velocity of change.
When applied to discrete-time systems—such as the layer-wise evolution of hidden states in LLMs—this continuous formulation naturally transitions into a summation:

\begin{equation}
S = \sum_{t=0}^{N-1} L_t, \quad L_t = T_t - U_t,
\end{equation}

where \(N\) is the total number of discrete steps (i.e., transformer layers), and \(L_t\) denotes the local Lagrangian at timestep \(t\). By defining kinetic and potential energies based on internal hidden state dynamics, we extend the classical Lagrangian framework to abstract reasoning paths in language models.

\subsection{CoT-Kinetics}

We define \( q_t \in \mathbb{R}^d \) as the average hidden representation of CoT-relevant tokens at layer \( t \), forming a discrete trajectory \( \{q_t\} \) across layers. Analogous to velocity and acceleration in physical systems, we define semantic dynamics as:

\begin{equation}
\dot{q}_t := v_t = q_{t+1} - q_t, \quad
\ddot{q}_t := a_t = q_{t+1} - 2q_t + q_{t-1},
\end{equation}

Both semantic derivatives are normalized by the total displacement between initial and final states \((q_0, q_N)\) to ensure scale-invariant dynamics across varying input complexities.

We then instantiate the discrete Lagrangian formalism by constructing a layerwise Lagrangian \(L_t\) as:
\begin{equation}
L_t = T_t - U_t := T_t^{(1)} + T_t^{(2)} - \gamma \cdot U_t,
\quad
S = \sum_{t=0}^{N-1} L_t,
\end{equation}

where \(T_t^{(1)} = \|\dot{q}_t\|\) captures the \textbf{semantic momentum energy}, quantifying forward representational dynamics, and 
\(T_t^{(2)} = \|\ddot{q}_t\|\) reflects the \textbf{semantic curvature energy}, characterizing local correction behaviors within the reasoning path.


==> sections/rel.tex <==
\section{Related Work}

\textbf{Large Reasoning Models (LRMs):} 
Comparing with LLMs, LRMs have demonstrated that extending the reasoning process can substantially enhance model inference performance. 
For example, \texttt{OpenAI-o1}~\cite{openai2024openaio1card}, \texttt{Qwen-QwQ}~\cite{qwq32b} and \texttt{DeepSeek-R1}~\cite{deepseekai2025deepseekr1incentivizingreasoningcapability} explicitly perform CoT reasoning by constructing an intermediate reasoning trajectory trying to justify the final answer~\cite{wei2023chainofthoughtpromptingelicitsreasoning}. LRMs show to be effective in domains requiring complex logical deduction, such as mathematics and programming~\cite{chen2023theoremqatheoremdrivenquestionanswering,cobbe2021gsm8k,hendrycks2021measuringmassivemultitasklanguage,shi2022languagemodelsmultilingualchainofthought,wang2024mmluprorobustchallengingmultitask,talmor-etal-2019-commonsenseqa}.
Unlike conventional LLMs, which produce an answer in a single forward pass guided by shallow heuristics, LRMs follow an explicit “think‑then‑answer” routine~\cite{deepseekai2025deepseekr1incentivizingreasoningcapability,openai2024openaio1card,qwq32b,geminiteam2025geminifamilyhighlycapable,muennighoff2025s1simpletesttimescaling}. They first enclose a CoT segment between special tokens (e.g., \texttt{<think>}…\texttt{</think>}) and repeatedly update internal representations while attending to these intermediate tokens; They generate the final answer only after completing the step-by-step deliberation process.

Current efforts to evaluate the overall output quality of an LRM can be broadly categorized into external and internal assessment methods, which are separately reviewed as follows.

\textbf{External Assessment:}
This type of assessment methods relies on supervision signals external to the model, such as linear probing techniques~\citep{wang2025thoughtprobe}, additional annotations or knowledge bases~\citep{li2023makinglargelanguagemodels, nguyen2024directevaluationchainofthoughtmultihop}, and proxy models~\citep{he2025largelanguagemodelsdetect}.
For example, \cite{kadavath2022languagemodelsmostlyknow} leverages the instruction-following capabilities of LLMs, enhanced by RLHF~\citep{ouyang2022traininglanguagemodelsfollow}, to generate confidence scores through carefully crafted prompts.
This paradigm encompasses a variety of general methodologies that directly elicit confidence estimates from LLMs via multi-stage pipelines, as broadly evaluated in~\citep{lin2022teachingmodelsexpressuncertainty, tian2023justaskcalibrationstrategies}.
\cite{manakul2023selfcheckgptzeroresourceblackboxhallucination} further investigates this approach by prompting GPT-3 to generate biographical passages from the WikiBio dataset and manually annotating the factuality of the generated content.
Similarly, the PSA pipeline~\citep{xiong2024llmsexpressuncertaintyempirical} estimates confidence by perturbing prompts~\citep{gao2024spuqperturbationbaseduncertaintyquantification} to produce multiple outputs and subsequently measuring their consistency.
However, these methods typically require access to ground-truth labels, external resources, or auxiliary models, limiting their generalizability in real-world scenarios where such information may be unavailable or impractical to obtain. This limitation motivates the exploration of a label-free, model-internal evaluation strategies.


\textbf{Internal Assessment:}
This type of assessment methods leverage the internal states obtained from the model its own, such as hidden representations~\citep{wang2025latentspacechainofembeddingenables} or uncertainty-based signals~\citep{shih2023longhorizontemperaturescaling, Huang_2025, si2023promptinggpt3reliable}, to infer the reliability of its output without relying on external supervision. While this direction alleviates the dependence on external labels and models, most existing internal assessment approaches still evaluate the output holistically, without explicitly disentangling the reasoning trajectory from the final answer. As a result, the correctness of the final answer inevitably introduces bias, masking deficiencies in the reasoning process itself. Consequently, these methods fail to properly assess the intrinsic quality of the model's reasoning, leaving a critical gap that motivates the need for more fine-grained evaluation frameworks.

\textbf{Summary:}
Comparing to the two types of existing methods, our {CoT-Kinetics} energy modeling approach improves the state-of-the-art solutions on the following two key aspects. 
First of all, CoT-Kinetic energy extracts the reasoning part out of the overall output answer and can explicitly assess the soundness of the reasoning part without any external information. Note that previous studies~\citep{wang2024chain, osti_10463284, turpin2023languagemodelsdontsay} have shown that flawed reasoning can yield correct answers. Hence, the capability able to independently assess the reasoning part is crucial~\citep{nguyen2024directevaluationchainofthoughtmultihop}, while none of the existing methods can do that. 
Second, techniques used to establish the CoT-Kinetics energy indeed overcome the deficiency of the existing modeling approaches. CoT-Kinetics energy offers a more principled modeling of the reasoning process and  gives a logical scoring capability to assess the overall quality of the overall output answers, surpassing all existing methods substantially.






